Efficient Differentially Private Secure Aggregation for Federated Learning via Hardness of Learning with Errors

Federated machine learning leverages edge computing to develop models from network user data, but privacy in federated learning remains a major challenge. Techniques using differential privacy have been proposed to address this, but bring their own challenges -- many require a trusted third party or else add too much noise to produce useful models. Recent advances in \emph{secure aggregation} using multiparty computation eliminate the need for a third party, but are computationally expensive especially at scale. We present a new federated learning protocol that leverages a novel differentially private, malicious secure aggregation protocol based on techniques from Learning With Errors. Our protocol outperforms current state-of-the art techniques, and empirical results show that it scales to a large number of parties, with optimal accuracy for any differentially private federated learning scheme.

==> ces-macros.tex <==
\RequirePackage{ifthen}

\renewcommand{\TirName}[1]{\textsc{#1}}

% !!! removed to build OOPSLA
% \renewcommand{\thetheorem}{\thesection.\arabic{theorem}}
% \renewcommand{\thelemma}{\thesection.\arabic{lemma}}
% \renewcommand{\theexample}{\thesection.\arabic{example}}
% \renewcommand{\thedefinition}{\thesection.\arabic{definition}}
% \renewcommand{\theproposition}{\thesection.\arabic{proposition}}
% \renewcommand{\thecorollary}{\thesection.\arabic{corollary}}

% !!! removed to build OOPSLA
% \numberwithin{theorem}{section}
% \numberwithin{lemma}{section}
% \numberwithin{example}{section}
% \numberwithin{definition}{section}
% \numberwithin{proposition}{section}
% \numberwithin{corollary}{section}

% !!! removed to build APLAS
% \ifthenelse{\equal{\theoremdefns}{0}}
% {
% \newtheorem{theorem}{Theorem}[section]
% \newtheorem{definition}[theorem]{Definition}
% \newtheorem{corollary}[theorem]{Corollary}
% \newtheorem{example}[theorem]{Example}
% \newtheorem{lemma}[theorem]{Lemma}
% \newtheorem{proposition}[theorem]{Proposition}
% \newenvironment{proof}{\noindent\textit{Proof. }}{}
% % \newcommand{\qed}{$\Box$}
% \def\squareforqed{\hbox{\rlap{$\sqcap$}$\sqcup$}}
% \def\qed{\ifmmode\squareforqed\else{\unskip\nobreak\hfil
% \penalty50\hskip1em\null\nobreak\hfil\squareforqed
% \parfillskip=0pt\finalhyphendemerits=0\endgraf}\fi}
% }
% {}

% \ifthenelse{\equal{\theoremdefns}{1}}
% {
% \newtheorem{theorem}{Theorem}
% \newtheorem{definition}{Definition}
% \newtheorem{corollary}{Corollary}
% \newtheorem{example}{Example}
% \newtheorem{lemma}{Lemma}
% \newtheorem{proposition}{Proposition}
% \def\squareforqed{\hbox{\rlap{$\sqcap$}$\sqcup$}}
% \def\qed{\ifmmode\squareforqed\else{\unskip\nobreak\hfil
% \penalty50\hskip1em\null\nobreak\hfil\squareforqed
% \parfillskip=0pt\finalhyphendemerits=0\endgraf}\fi}
% }
% {}

\newcommand{\cesnote}[1]{\textit{(#1 -- c.e.s.)}}
\newcommand{\snote}[1]{{\small \textbf{\textit{(#1 -- Scott)}}}}
\newcommand{\dcdnote}[1]{{\color{magenta}\it (#1 -- {d.c.d.})}}

%\def\longhtobpa#1{\text{BPA}(#1)}
%\def\shorthtobpa#1{#1} % ignore BPA translation in short version

%\long\def\eatit#1{}
%\long\def\spititback#1{#1}
%\long\def\spitsmaller#1{{\def\formulasize{\scriptsize} {\scriptsize #1}}}
%\def\shortversion{\def\condensed{\spititback} \def\cut{\eatit}\def\htobpa{\shorthtobpa}}
%\def\longversion{\def\condensed{\eatit} \def\cut{\spititback}\def\htobpa{\longhtobpa}}
%\def\shortversionshowlongs{\def\condensed{\spititback} \def\cut{\spitsmaller}}
%\shortversion


\newcommand{\colfigurebox}[5]
{
        \begin{figure}
        \begin{center}
        \framebox[#1]{
                \begin{minipage}{#2}
                \footnotesize
                \vspace{2mm}
                #5
                \vspace{1mm}
                \end{minipage}
                \normalsize
        }
        \caption{#4} 
        \label{#3}
        \end{center}
        \end{figure}
}

\newcommand{\figurebox}[5]
{
        \begin{figure*}
        \begin{center}
        \framebox[#1]{
                \begin{minipage}{#2}
                \footnotesize
                \vspace{2mm}
                #5
                \vspace{1mm}
                \end{minipage}
                \normalsize
        }
        \caption{#4} 
        \label{#3}
        \end{center}
        \end{figure*}
}

%%%%% dduct %%%%%%
\newcommand{\dduct}[2]{
\ensuremath{
\renewcommand{\arraystretch}{1.3}
        \begin{array}[b]{c}
                #1\\\hline
                #2
        \end{array}
\renewcommand{\arraystretch}{1}
}
}
%%%%%%%%%%%%%%%%%%%

\newcommand{\algtab}[1]
{
\vspace*{-3mm}
\begin{tabbing}
\hspace*{12mm}\=\hspace{9mm}\=\hspace{9mm}\=\hspace{6mm}\=\hspace{6mm}\=
\hspace{6mm}\=\\\newcommand{\cmnts}{\noindent\textbf{Comments\hspace{2mm}}}
#1
\end{tabbing}
}
\newcommand{\lt}{\left\{}
\newcommand{\rt}{\right\}}
\newcommand{\Lt}{\left\{\!\!\right.}
\newcommand{\Rt}{\left.\!\!\right\}}
\newcommand{\const}{\mathbf{c}}
\newcommand{\heading}[1]{\noindent\textbf{#1\ \  }}

\newcommand{\schemecomp}[3]{#1\vdash^i#2\preccurlyeq#3}

\newcommand{\Estep}{\rightarrow}
\newcommand{\instance}{\preccurlyeq}
\newcommand{\geninstance}{\trianglelefteq}
\newcommand{\gen}{\mathit{gen}}
\newcommand{\genvars}{\mathit{genvars}}

\newcommand{\iruleone}{\textsc{Sub$^\instance$}}
\newcommand{\iruletwo}{$(\preccurlyeq\!\forall)$}
\newcommand{\irulethree}{$(\forall\!\preccurlyeq)$}

%\newcommand{\seclang}{\lambda_{\text{\rm sec}}}
%\newcommand{\setlang}{\lambda_{\text{\rm set}}}
\newcommand{\pinit}{\ensuremath{p_0}}
\newcommand{\reduce}{\leadsto}
\newcommand{\ctxreduce}{\rightarrow}
%\newcommand{\eqdefn}{=_{\scriptscriptstyle{\mathit{def}}}}
\newcommand{\subn}{\psi}
\newcommand{\subndefn}[1]{[#1]}
\newcommand{\restrict}[2]{{#1}\!\mid_{#2}}
\newcommand{\rrow}[2]{\lt \drow{r}{#1}{#2} \rt}
\newcommand{\refcell}{\mathrm{ref}}
\newcommand{\tref}{\mathrm{ref}}
\newcommand{\hmxconfig}[2]{#1/#2}
%\newcommand{\store}{\varsigma}
\newcommand{\rangevec}[3]{#1^{\hspace{4pt}#2 \in \setdefn{1,\ldots,#3}}}
\newcommand{\initenv}{\Delta}
\newcommand{\extend}[3]{#1[#2 \mapsto #3]}
\newcommand{\gdesc}[1]{\text{\textit{#1}}}
%\newcommand{\loc}{l}
\newcommand{\setdefn}[1]{\lt#1\rt}
\newcommand{\deref}{\,!}
\newcommand{\assignfn}[1]{{:=}_{#1}}
%\renewcommand{\eabs}[3]{\lambda\langle#1\rangle #2 . #3 }
\newcommand{\credentials}{\mathcal{A}}
\newcommand{\constrain}[2]{#1\!\mid_{#2}}
\newcommand{\subrule}{\TirName{Sub}}
\newcommand{\varrule}{\TirName{Var}}
\newcommand{\locrule}{\TirName{Loc}}
\newcommand{\absrule}{\TirName{Abs}}
\newcommand{\apprule}{\TirName{App}}
\newcommand{\letrule}{\TirName{Let}}
\newcommand{\assignrule}{\TirName{Assign}}
\newcommand{\construle}{\TirName{Const}}
\newcommand{\refrule}{\TirName{Ref}}
\newcommand{\derefrule}{\TirName{Deref}}
\newcommand{\forallelim}{\TirName{$\forall$ Elim}}
\newcommand{\forallintro}{\TirName{$\forall$ Intro}}
\newcommand{\configrule}{\TirName{Config}}
\newcommand{\allv}{\beta}
\newcommand{\svar}{\alpha}
\newcommand{\vvec}{\bar{\allv}}
\newcommand{\tvec}{\bar{\tau}}
\newcommand{\existsC}[2]{\exists #1 . #2}
\newcommand{\rename}{\varrho}
\newcommand{\metaj}{\mathcal{J}}
\newcommand{\eass}[1]{\mathord{:=}\,#1}
\newcommand{\eassign}[2]{\mathord{:=}\,#1\,#2}
\newcommand{\cesqed}{}
\newcommand{\sys}{\ensuremath{\system{1}{=}}}
\newcommand{\etal}{\emph{et al.}}
%\newcommand{\enabler}{\mathrm{enable}_r}
%\newcommand{\requirer}{\mathrm{require}_r}
\newcommand{\defeq}{\triangleq}
\newcommand{\bestAttc}{\text{\it tryKill'}}
\newcommand{\labs}[2]{\lambda #1 . #2}
\newcommand{\menabler}{\ensuremath{{\text{\it maybeEnable}}_r}}
\newcommand{\action}{\text{\it action}}
\newcommand{\tin}{\tpre}
\newcommand{\tout}{\tabs}
\newcommand{\allsett}{\urow{\tin}}
\newcommand{\nonesett}{\urow{\tout}}
\newcommand{\snext}{\tnext}
%\newcommand{\fielduk}[2]{\stackrel{\;#2}{#1}}
\newcommand{\fielduk}[2]{#1:#2}
\newcommand{\fieldint}[1]{\fielduk{#1}{\tin}}
\newcommand{\fieldoutt}[1]{\fielduk{#1}{\tout}}
%\newcommand{\fieldint}[1]{\dot{#1}}
%\newcommand{\fieldoutt}[1]{\bar{#1}}
\newcommand{\srow}[3]{\fielduk{#1}{#2}\snext#3}
\newcommand{\trule}[1]{\textsc{#1}}
\newcommand{\etrue}{\fpkeyword{true}}
\newcommand{\efalse}{\fpkeyword{false}}
\newcommand{\boolt}{\textit{bool}}
\newcommand{\unitt}{\textit{unit}}
\newcommand{\unroll}[2]{\circlearrowright_{#1}#2}
\newcommand{\acclang}{\ensuremath{\lambda_{\mathrm{trace}}}}
\newcommand{\histlang}{\acclang}
%\newcommand{\stacklang}{\ensuremath{\lambda_{\mathrm{trace}}}}
\newcommand{\stacklang}{\ensuremath{\acclang^{\hstack}}}
\newcommand{\hist}{\theta}
\newcommand{\hconfig}[2]{#1,#2}
\newcommand{\hlog}[2]{#1;#2}
\newcommand{\boolinterp}[1]{\cod{#1}_\mathrm{bool}}
\newcommand{\squeeze}[1]{\hat{#1}}
\newcommand{\bigsqueeze}[1]{\widehat{#1}}
\newcommand{\scontextfn}{\text{context}}
\newcommand{\scontext}[2]{\scontextfn_{#1}(#2)}
\newcommand{\slength}{\text{length}}
\newcommand{\fdepth}{\text{fdepth}}
\newcommand{\sframefn}{\text{frame}}
\newcommand{\sframe}[2]{\sframefn_{#1}(#2)}
\newcommand{\hjudge}[4]{#1, #2 \vdash #3 : #4}
\newcommand{\hcijudge}[5]{#1, #2 \vdash_{#3} #4 : #5}
\newcommand{\hijudge}[4]{#1, #2 \vdash_{W} #3 : #4}
\newcommand{\hcjudge}[5]{#1, #2, #3 \vdash #4 : #5}
\newcommand{\lhjudge}[5]{#1, #2, #3 \vdash #4 : #5}
\newcommand{\gchjudge}[5]{#1, #2, #3 \vdash #4 : #5}
\newcommand{\labinferrule}[3]{\inferrule*[right=\scriptsize#3]{#1}{#2}}
\newcommand{\linfer}[3]{\inferrule*[right=\textsc{\scriptsize#3}]{#1}{#2}}
\newcommand{\Labinferrule}[3]{\inferrule*[Right=\scriptsize#3]{#1}{#2}}
\newcommand{\singleton}[1]{\tset{#1}}
\newcommand{\tsetp}[1]{\tset{\cdot#1\cdot}}
\newcommand{\arrowt}[1]{\xrightarrow{#1}}
\newcommand{\arrowht}[3]{#1 \arrowt{#2} #3}
\newcommand{\HC}{\mathit{HC}}
\newcommand{\evsig}{\Sigma}
\newcommand{\logbook}{\varsigma}
\newcommand{\logbookt}{\Sigma}
\newcommand{\hid}{\iota}
\newcommand{\hdecl}[2]{\fpkeyword{history }#1\text{ in }#2}
\newcommand{\lev}[1]{\ev_{#1}}
\newcommand{\lcheck}[2]{#1_{#2}}
\newcommand{\hsubn}{\psi}
\newcommand{\evpush}{\mathrm{push}}
\newcommand{\evpop}{\mathrm{pop}}
\newcommand{\stackify}{\mathit{stackify}}
\newcommand{\inspect}{\mathit{inspect}}
\newcommand{\fresh}[1]{#1 \text{ fresh}}
\newcommand{\pdistinct}[1]{#1 \text{ p-distinct}}
%\newcommand{\enew}[2]{\fpkeyword{new}\ #1\ \fpkeyword{in}\ #2}
\newcommand{\enew}[2]{\fpkeyword{new}\ #1\ \fpkeyword{in}\ #2}
\newcommand{\sexists}[2]{\exists #1 . \singleton{#2}}
\newcommand{\gcvar}{\zeta}
\newcommand{\gcvvec}{\bar\zeta}
\newcommand{\gcarrowt}[4]{\nabla #1 . #2 \xrightarrow{#3} #4}
\newcommand{\variantt}[1]{[#1]}
%\newcommand{\kind}[2]{#1:#2}
\newcommand{\ksingle}{\textit{Sing}}
\newcommand{\khistory}{\textit{Eff}}
%\newcommand{\kgcsingle}{\text{\emph{Single}}_{\gcvar}}
\newcommand{\ktype}{\textit{Type}}
\newcommand{\fvgc}[1]{\text{\rm fv}_\gcvar(#1)}
%\newcommand{\tvset}[1]{\mathcal{V}_{#1}}
\newcommand{\hvvec}{\bar{h}}
\newcommand{\cvec}{\bar{c}}
\newcommand{\gchist}[2]{\nabla #1 . #2}
\newcommand{\truncate}[1]{#1\backslash_{\mu}}
\newcommand{\trace}{\vartheta}
\newcommand{\Trace}{\Theta}
\newcommand{\halt}{\fpkeyword{halt}}
\newcommand{\diverge}{\uparrow}
\newcommand{\aftrans}[1]{\stackrel{#1}{\leadsto}}
\newcommand{\intersect}{\mathit{intersect}}
\newcommand{\demand}{\mathit{demand}}
\newcommand{\hfloor}[1]{\lfloor #1 \rfloor}
\newcommand{\ncod}[2]{\lfloor #2 \rfloor_{#1}}
\newcommand{\hbasis}{\mathit{basis}}
\newcommand{\hbases}{\mathit{bases}}
\newcommand{\metalet}[3]{\text{let}\,#1=#2\,\text{in}\,#3}
\newcommand{\metaite}[3]{\text{if}\,#1\,\text{then}\,#2\,\text{else}\,#3}
\newcommand{\ltrans}[1]{\xrightarrow{#1}}
\newcommand{\gcltrans}[2]{\xrightarrow{#2}_{#1}}
%\newcommand{\acclangver}[1]{\lambda_{\mathrm{trace}}^{#1}}
\newcommand{\bpatrans}[2]{{\text{BPA}(#1,#2) }}
%\newcommand{\evkeyword}[1]{\scriptstyle{\mathbf{#1}}}
\newcommand{\evkeyword}[1]{{\mathrm{#1}}}
\newcommand{\evenable}[1]{\mathrm{enable}_#1}
\newcommand{\phiinsp}{\phi_\text{inspect}}
\newcommand{\phiinspect}[1]{\phi_{\text{inspect,}#1}}
\newcommand{\phienable}[1]{\phi_{\text{enable,}#1}}
\newcommand{\phiamplify}[1]{\phi_{\text{amplify,}#1}}
\newcommand{\evinspect}[1]{\phiinspect{#1}}
\newcommand{\evamplify}[1]{\fpkeyword{amplify}_{#1}}
\newcommand{\evdemand}[1]{\fpkeyword{demand}_{#1}}
\newcommand{\evmgr}{\fpkeyword{mgr}}
\newcommand{\evacct}{\fpkeyword{acct}}
\newcommand{\evcrit}{\fpkeyword{crit}}
%\newcommand{\trans}[1]{\langle #1 \rangle}
\newcommand{\trans}[1]{( #1 )}
%\newcommand{\alltrans}[1]{[ #1 ]}
\newcommand{\nowlab}{\mathrm{Now}}
\newcommand{\pc}[1]{#1\!\!\downarrow}
\newcommand{\cvar}{\chi}
\newcommand{\existsend}{\trans{\mathrm{Now}}}
%\newcommand{\allend}{[ \mathrm{Now} ]}
\newcommand{\evdelim}{\circ}
\newcommand{\evldelim}{\rhd}
\newcommand{\evrdelim}{\lhd}
\newcommand{\muenable}[1]{\phi_{\text{enable-ok,#1}}}
\newcommand{\muinspect}[1]{\phi_{\text{inspect-ok,#1}}}
\newcommand{\muamplify}{\text{amplify}}
\newcommand{\mudemand}{\text{demand}}
\newcommand{\phidemand}[1]{\phi_{\text{demand},#1}}
\newcommand{\phidemandone}[1]{\phi_{\text{demand1},#1}}
\newcommand{\phidemandtwo}[1]{\phi_{\text{demand2},#1}}
\newcommand{\jsicheck}{\text{checkit}}
\newcommand{\jsienable}{\text{enableit}}
\newcommand{\filewpriv}{{r{:}\evkeyword{filew}}}
\newcommand{\htoX}{\Psi}
\newcommand{\mumu}{\mbox{\boldmath{$\mu$}}}
\newcommand{\munu}{\mbox{\boldmath{$\nu$}}}
\newcommand{\pinterp}{\Pi}
\newcommand{\staticpinterp}{\Pi_{\mu}}
\newcommand{\muinterp}[2]{\llbracket#1\rrbracket^{#2}}
\newcommand{\preprocess}{\text{pp}}
\newcommand{\emptystack}{\text{nil}}
\newcommand{\dotstack}{\varsigma}
\newcommand{\hframe}{\mathit{frame}}
\newcommand{\systemp}{{p{:}\evkeyword{system}}}
\newcommand{\acctp}{{p{:}\evkeyword{acct}}}
\newcommand{\Poccurs}[1]{\text{occurs}(#1)}
\newcommand{\jgmt}{\mathcal{J}}
\newcommand{\erase}{\text{erase}_\hist}
\newcommand{\terase}{\text{erase}_H}
\newcommand{\stjudge}[3]{#1 \vdash #2 : #3}
\newcommand{\ltsV}{V}
\newcommand{\muentails}[1]{\Vdash_{#1}}
\renewcommand{\implies}{\Rightarrow}
\newcommand{\simplecheck}{\phi}
\newcommand{\contains}{\sqsupseteq}
\newcommand{\stacked}[1]{{\cdot{#1}\cdot}}
\newcommand{\cons}[2]{\ensuremath{#1\!::\!#2}}
\newcommand{\hstack}{\ensuremath{\mathtt{S}}}
\newcommand{\hists}{\mathcal{H}}
\newcommand{\flowsto}{\sqsubseteq}
\newcommand{\closure}{\mathit{close}}
\newcommand{\hclosure}{\mathit{hclose}}
\newcommand{\mgu}{\mathit{MGS}}
\newcommand{\unifysoln}{\mathit{soln}}
\renewcommand{\scheme}[3]{\forall#1.#3/#2}
\newcommand{\po}{\preccurlyeq}
\newcommand{\hlt}{\preccurlyeq}
\newcommand{\monot}{\hat{\tau}}
\newcommand{\interp}{\rho}
\newcommand{\unify}{\mathit{unify}}
\newcommand{\subtype}[2]{#1\, \flowsto\, #2}
\newcommand{\hextract}{\mathit{hextract}}
\newcommand{\hextractC}{\mathit{hextract}_{C}}
\newcommand{\sextract}{\mathit{sextract}}
\newcommand{\ctrans}{\leadsto_\mathit{close}}
\newcommand{\ctransctx}{\rightarrow_\mathit{close}}
\newcommand{\close}{\mathit{close}}
\newcommand{\hclose}{\mathit{hclose}}
\newcommand{\bounds}{\mathit{bounds}}
\newcommand{\hsplit}{\mathit{hsplit}}
\newcommand{\cok}[1]{\vdash #1 : \mathit{ok}}
\newcommand{\habstract}[2]{\mathit{abstract}(#1,#2)}
\newcommand{\HX}{\mathit{HX}}
\newcommand{\mut}[2]{\mu #1 . #2}

\def\with{\ \mathit{with}\ }
\def\requiring{\ \mathit{requiring}\ }
\def\nothing{\mathit{nada}}
\def\ev{\mathit{e\!v}}
\def\Ev{\mathit{E\!\!V}}
\def\check{\fpkeyword{check}\ }
\def\unit{\fpkeyword{unit}}
\def\emptyhistory{\epsilon}
\def\effarrow#1{\stackrel{#1}{\rightarrow}}
\def\effpredarrow#1#2{\overset{\scriptscriptstyle #1}{\underset{\scriptscriptstyle #2}\rightarrow}}
\newcommand{\treeltfin}{\preccurlyeq_{\text{fin}}}
\newcommand{\treelt}{\preccurlyeq}
%\newcommand{\arrowht}[3]{#1\xrightarrow{#2} #3}
\newcommand{\nat}{\mathbb{N}}
\newcommand{\Trees}{\mathbb{T}}
\newcommand{\tree}{\varphi}
\newcommand{\treepath}{\pi}
\newcommand{\cut}[2]{#1\!\mid\!_{#2}}
\newcommand{\sig}{\varsigma}
\newcommand{\chk}{\phi}
\newcommand{\cardinal}[1]{|#1|}
\newcommand{\strace}{\varsigma}
\newcommand{\sctx}{\mathrm{sctx}}
\newcommand{\sctxs}{\mathrm{sctxs}}
\newcommand{\scod}[1]{\llparenthesis\,#1\,\rrparenthesis}
\newcommand{\cdummy}{c_{\mathrm{dummy}}}
\newcommand{\historify}[1]{\lfloor#1\rfloor}

\def\Subn{\Phi}
\def\merge{\mathit{M}}
\def\smerge{\mathit{M}_\subn}
\def\hmerge{\mathit{M}_H}
\def\tmerge{\mathit{M}_\tau}
\def\gmerge{\mathit{M}_\Gamma}
\def\humerge{\mathit{merge}_H^0}
\def\rmnabla{\not{\!\nabla}}
\def\mudnf{\mu\mathit{dnf}}
\def\zeight{\mathit{Z\mbox -8}}

\newcommand{\ctype}[2]{#1/#2}
\newcommand{\strip}[1]{\lfloor#1\rfloor}
\newcommand{\htobpa}[1]{\text{BPA}(#1)}
\newcommand{\Cset}[1]{\mathit{set}(#1)}
\newcommand{\clashes}{\asymp}

%% NEW HOOKADVICE MACROS BELOW
\long\def\cnote#1{{\small\textbf{\textit{\color{red}(*#1 -- Chris*)}}}}%% NEW HOOKADVICE MACROS BELOW
\long\def\dnote#1{{\small\textbf{\textit{\color{blue}(*#1 -- David*)}}}}%% NEW HOOKADVICE MACROS BELOW
\long\def\tnote#1{{\small\textbf{\textit{\color{violet}(*#1 -- Tim*)}}}}
\long\def\jnote#1{{\small\textbf{\textit{\color{brown}(*#1 -- Joe*)}}}}
\long\def\xl#1{{\small\textbf{\textit{\color{blue}(*#1 -- Christelle*)}}}}
%\long\def\cnote#1{\marginpar{CS}{\small \ \ $\langle\langle\langle$\
%{#1 - CS}\
%    $\rangle\rangle\rangle$\ \ }} 
\newcommand{\openchan}{\fpkeyword{open}}
\newcommand{\chanread}[1]{#1.\fpkeyword{read}}
\newcommand{\chansubj}[1]{#1.\fpkeyword{subject}}
\newcommand{\chanwrite}[2]{#1.\fpkeyword{write}(#2)}
\newcommand{\subj}{\texttt{s}}
\newcommand{\subjs}{\bar{\subj}}
\newcommand{\subjvar}{\gamma}
\newcommand{\subjvars}{\bar{\alpha}}
\newcommand{\chan}{\mathbf{c}}
\newcommand{\exhm}[3]{\exists #1 . \{ #2, #3 \}}
\newcommand{\sett}[1]{\{ #1 \}}
\newcommand{\intt}{\mathit{int}}
\newcommand{\chant}[1]{\mathit{chan}[#1]}
%\newcommand{\chant}{\mathit{chan}}
\newcommand{\priv}{\pi}
%\newcommand{\hook}[2]{#1.\fpkeyword{auth}(#2)}
\newcommand{\hook}[1]{\fpkeyword{hook}(#1)}
\newcommand{\taintint}[1]{\intt_{#1}}
\newcommand{\taintv}[2]{{#1}\cdot{#2}}
\newcommand{\authev}[2]{#1\ \fpkeyword{requires}\ #2}
\newcommand{\authevq}[2]{#1\ \fpkeyword{requires}^?\ #2}
\newcommand{\indflowev}[2]{#1 \hookrightarrow #2}
\newcommand{\flowev}[2]{#1 \leadsto #2}
\newcommand{\flowevq}[2]{#1 \leadsto^? #2}
\newcommand{\deltaty}[4]{#1 \rightarrow \Delta #2 . #4,#3}
\newcommand{\fixty}[3]{#1 \rightarrow #2,#3}
\newcommand{\svec}{\bar{\subj}}
\newcommand{\freesubs}[1]{\mathrm{subjects}(#1)}
\newcommand{\subjt}{\varsigma}
\newcommand{\subjts}{\bar{\subjt}}
\newcommand{\tjudge}[5]{#2 \vdash_{#1} #4 : #5 \cdot #3}
\newcommand{\redx}{\rightarrow}
\newcommand{\redxs}{\redx^{*}}
\newcommand{\chanv}[1]{\langle #1 \rangle}
\newcommand{\acp}{\mathcal{A}}
\newcommand{\ifp}{\mathcal{F}}
\newcommand{\hooklang}{\Lambda_{\mathit{hook}}}
\newcommand{\rv}{\mathit{rv}}
\newcommand{\ksubject}{\textit{Subj}}
\newcommand{\kpc}{\textit{PC}}
\newcommand{\pow}[1]{\mathit{pow}(#1)}


\newcommand{\store}{\Sigma}
\newcommand{\loc}{\ell}
\newcommand{\eref}[1]{\fpkeyword{ref}\ #1}
\newcommand{\reft}[1]{\fpkeyword{ref}\ #1}
\renewcommand{\initenv}{\mathcal{E}}
\renewcommand{\subn}{\varrho}
\newcommand{\readpriv}{\mathbf{r}}
\newcommand{\writepriv}{\mathbf{w}}
\newcommand{\closeacp}{\mathrm{close}}

\newcommand{\fvar}{\alpha}
\newcommand{\flab}{\ell}
\newcommand{\fty}{\phi}
\newcommand{\flabty}[2]{#1^{#2}}
\newcommand{\recty}[1]{\{ #1 \}}
\newcommand{\labof}{\mathit{lab}}
\newcommand{\lattice}{\mathcal{L}}
\newcommand{\latel}{p}
\newcommand{\hilab}{\fpkeyword{hi}}
\newcommand{\lolab}{\fpkeyword{lo}}
\newcommand{\flowmap}{\mathcal{K}}
\newcommand{\subjlevels}{\flowmap_{\mathit{pol}}}
\newcommand{\ilab}{\subj}
\newcommand{\sle}{\preccurlyeq}
%\newcommand{\declass}[2]{\lfloor#2\rfloor_{#1}}
\newcommand{\declass}[2]{#2\!\downarrow_{#1}}
\newcommand{\halfmeet}[2]{#1\,\sqcap_{#2}}
\newcommand{\readf}{\mathrm{read}}
\newcommand{\writef}{\mathrm{write}}
\newcommand{\oklab}{\mathrm{ok}}
\newcommand{\badlab}{\mathrm{bad}}
\newcommand{\assignev}[2]{#1 \leftarrow #2}
\newcommand{\shookev}[1]{\mathit{check}(#1)}
\newcommand{\tr}{\theta}
\newcommand{\stepone}{\mathit{step}}
\newcommand{\steptwo}{\bar{\stepone}}
\newcommand{\stepthree}{\hat{\stepone}}
%\newcommand{\traceinterp}[1]{\llbracket #1 \rrbracket}
\newcommand{\hooktruncate}[1]{\lfloor #1 \rfloor}
\newcommand{\acl}{\mathcal{A}}
\newcommand{\mi}[1]{\mathit{#1}}
\newcommand{\ttt}[1]{\ensuremath{\mathtt{#1}}}

\newcommand{\ourprot}{\ensuremath{\mathrm{FLDP}}\xspace}


==> threat_models.tex <==
\section{Background: Balancing Trust and Accuracy}

\begin{table*}\label{fig-comparison}
  \begin{tabular}{|c||c|c|c|}
  \hline
  & \textit{Accuracy} & \textit{DP Third Party} & \textit{Honest Majority} \\
  \hline \hline
  \textbf{Centralized Model} & High & Yes, trusted & No\\
  \hline
  \textbf{Untrusted Servers Model} & N/A for FL & Yes, trusted non-colluding & Yes (servers)\\
  \hline  
  \textbf{\ourprot} & High & No & Yes (participants) \\ 
  \hline
  \textbf{Local Model} & Low & No & No \\
  \hline
\end{tabular}
    \caption{Comparison of Approaches to Federated Learning (FL) with DP}
\end{table*}




The general aim of our system is to perform federated learning at large scales with privacy. More specifically, we assume that federation participants possess confidential data that is used as input to a gradient descent algorithm, such that computed gradients are differentially private with respect to participant input data. As discussed above, DP is known to defend against various attacks such as membership inference \cite{DBLP:journals/corr/ShokriSS16,jayaraman2020revisiting}. Throughout this paper, we will use DP to refer specifically to $(\epsilon,\delta)$-DP since this is the most practical and well-studied approach in our setting. 

Previous work has explored similar challenges of conducting federated computations with differential privacy. The main points of comparison we consider in our proposed systems and evaluation are \emph{trust} and \emph{accuracy}. Definitions of accuracy depend on the nature of the performed computation, but we are mainly concerned with federated learning (FL) and thus model accuracy. The issue of trust can be framed in terms of which system elements are trusted and therefore vulnerable to compromise. Our goal is to obtain an improved balance of trust and accuracy, as compared to previous work.

In all systems there exist federation participants and an \emph{aggregator} who combines participant contributions to obtain a full model. Different systems explore different techniques to inject noise into models which affect both accuracy and vulnerability of the system. In a fully \emph{centralized} model that has been explored in existing work \cite{XXX}, the aggregator is a trusted third party who injects noise into participant data to obtain a model with DP. The accuracy of models obtained in this way is the best that is can be achieved with DP, but this approach has the drawback of complete trust in the third party aggregator, which we aim to eliminate.

Other previous work has explored a fully \emph{local} model, where participants compute model gradients on their own private inputs, and then add noise to the gradients locally to obtain differential privacy. These gradients are then shared with the aggregator, who combines them into a complete model which also enjoys differential privacy compositionally. This approach has the benefit of eliminating a trusted third party and any exposure of private data. However at scale it has the drawback of yielding extremely poor accuracy in the final model- as prior work has shown, accuracy with this technique scales disastrously with federation sizes \cite{wagh2020dpcryptography}.

An intermediate approach that we call the \emph{untrusted servers} model has been considered that begins to strike a balance between the local and global models \cite{10.1145/3318464.3380596}. Here, two or (a few) more third party servers perform a secure multi-party computation (MPC) protocol to add noise to encrypted participant data. This eliminates the need for a trusted third party in a sense, however the scheme requires these servers to be non-colluding in a so-called honest majority, which in the case of e.g.~two servers means that only one server needs to be compromised to undermine the scheme. Furthmore, their current system is not able to perform the breadth of computations necessary for federated learning, especially due to reliance on homomorphic encryption. \cnote{Probably need to say more about this last point.}

The aim of this paper is to propose, implement, and evaluate a new protocol, called $\ourprot$, for Federated Learning (FL) with Differential Privacy (DP). The $\ourprot$ protocol leverages large scale secure multi-party computation (MPC) to eliminate the need for any third party in DP computations while maintaining model accuracy. Our main research hypothesis is that our system can achieve significantly better accuracy than the local model, while eliminating any trusted third party as in the centralized model.

While a technical contribution of our work is significantly greater scaling of MPC protocols than previous state-of-the-art, full federation-scale MPC is practically infeasible using existing protocols. However, we observe that the standard technique of federated learning in \emph{minibatches} ensures tractable MPC group sizes with our innovations. Also, while completely general MPC computation (e.g.~evaluation of arithmetic circuits) is currently intractable at larger scales, we show that the computations needed
to support federated learning are more restricted and thus tractable. We focus our evaluation on the simulation of a large-scale federated learning task with differential privacy, and the accuracy of the model obtained through this simulation.

\subsection{Paper Overview} The aim of this paper is to propose, implement, and evaluatte a new protocol, called $\ourprot$, for Federated Learning (FL) with Differential Privacy (DP). The $\ourprot$ protocol is based on large scale secure multi-party computation (MPC) to achieve a balance of privacy, accuracy, and efficiency. We describe a complete implementation of the protocol, and a simulation of it running in minibatch sizes up to 1000 \cnote{an aspirational figure.}. We run a complete machine learning task, \cnote{brief description and citation here}. An evaluation of the accuracy of the model generated in our simulation demonstrates that the $\ourprot$ protocol is feasible for machine learning tasks. The simulation also demonstrates tractability of the approach up to the maximum tested minibatch size.

In more detail: In Section \ref{sec-core_protocols}, we discuss the underlying constituent MPC and DP protocols we use in $\ourprot$, which are based on direct or modified adaptations of previous work. In Section \ref{sec-jfl} we give a formal definition of the $\ourprot$ protocol, and describe how the constituent MPC and DP protocols support the full protocol. In Section \ref{sec-implementation} we describe our protocol implementation. This includes underlying network and communication architectures, and details about the deep learning algorithm, data, and methods employed. In Section \ref{sec-evaluation} we describe our experimental simulation methods, experiments, and evaluation metrics. This Section also includes evaluation results and discussion. We end with comments on related and future work in Section \ref{sec-conclusion}.


\cnote{Star topology DP: https://dl.acm.org/doi/10.1145/3029806.3029829}


==> threat_models_new.tex <==
\section{Background and Problem Statement}
\label{sec:overview}
\label{sec:problem}

% \begin{figure*}
%   \begin{tabular}{|c||c|c|c|}
%   \hline
%   & \textit{Accuracy} & \textit{Threat Model} & \textit{Ref.} \\
%   \hline \hline
%   \textbf{Centralized Model} & High & Fully trusted & No\\
%   \hline
%   \textbf{Untrusted Servers Model} & N/A for FL & Yes, trusted non-colluding & Yes (servers)\\
%   \hline  
%   \textbf{\ourprot} & High & No & Yes (participants) \\ 
%   \hline
%   \textbf{Local Model} & Low & No & No \\
%   \hline
% \end{tabular}
% \caption{Comparison of Approaches to Federated Learning (FL) with DP}
% \label{fig:approaches}
% \end{figure*}

\begin{table*}
  {
    \def\arraystretch{1.2}
  \begin{tabular}{|c||c|c|c|c|c|}
    \hline
    \textit{Reference} & \textit{Approach} & \textit{Accuracy} & \textit{Threat Model, Aggregator} & \textit{Threat Model, Participants} & \textit{Collusion Resistance}\\
    \hline \hline
    Abadi et al.~\cite{dpdl} & Central DP & High & Fully trusted (1 server) & N/A & 1 party\\
    \hline
    Bonawitz et al.~\cite{bonawitz2017aggregation} & Secure Aggregation & High & Semi-honest (1 server) & Semi-honest & 1 party\\
    \hline
    Jayaraman et al.~\cite{DBLP:conf/nips/JayaramanW0G18} & Garbled Circuits & High & Semi-honest (2 servers) & Semi-honest & 2 parties\\
    \hline
      Bhowmick et al.~\cite{bhowmick2018protection} & Local DP & Low & Malicious (1 server) & Malicious (all other parties) & $n$ parties \\
    \hline
    \rowcolor[RGB]{230,230,230}  \textbf{\ourprot} (ours) & Secret Sharing & High & Malicious (1 server) & Malicious (honest majority) & $n/2$ parties \\
    \hline
  \end{tabular}
  }
  \caption{Comparison of Threat Models for Differentially Private Deep Learning.}
  \label{fig:approaches}
\end{table*}

We study the problem of \emph{distributed differentially private deep learning without a trusted data curator}. Our setting includes a set of \emph{participants} (or data owners), each of whom holds some sensitive data, and an \emph{aggregator} who wishes to train a model using this data. The goal is to use the distributed data to train a differentially private model, without revealing any participant's data to any other participant or the aggregator.

\subsection{Technical Background \& Related Work}

\paragraph{Deep learning.}
Deep learning~\cite{goodfellow2016deep} attempts to train a neural network architecture $\mathcal{F}(\theta, \cdot)$ by training its \emph{parameters} (or \emph{weights}) $\theta$ in order to minimize the value of a \emph{loss function} $\mathcal{L}(\theta, \cdot)$ on the training data. Advances in deep learning have lead to significant gains in machine learning capabilities in recent years. Neural networks are typically trained via \emph{gradient descent}: each iteration of training calculates the gradient of the loss on a subset of the training data called a \emph{batch}, and the model parameters are updated based on the negation of the gradient.

Traditional deep learning techniques assume the training data is collected centrally; moreover, recent results suggest that trained models tend to memorize training data, and training examples can later be extracted from the trained model via \emph{membership inference attacks}~\cite{shokri2017membership, yeom2018privacy, carlini2019secret, jayaraman2020revisiting}. When sensitive data is used to train the model, both factors represent significant privacy risks to data owners.

\paragraph{Federated learning.}
Federated learning is a family of techniques for training deep neural networks without collecting the training data centrally. In the simplest form of federated learning (also called \emph{distributed SGD}), each participant computes a gradient locally and sends the gradient (instead of the training data) to the aggregator. The aggregator averages the gradients and updates the model. More advanced approaches compute gradients in parallel to reduce communication costs; Kairouz et al.~\cite{kairouz2019advances} provide a survey.

\paragraph{Differentially private deep learning.}
Differential privacy~\cite{dwork2014algorithmic} is a rigorous privacy framework that provides a solution to the problem of privacy attacks on deep learning models. Achieving differential privacy typically involves adding noise to results to ensure privacy. Abadi et al.~\cite{dpdl} introduced an algorithm for training deep neural networks with differential privacy by adding noise to gradients before each model update. Subsequent work has shown that this approach provides strong privacy protection, effectively preventing membership inference attacks~\cite{yeom2018privacy, carlini2019secret, jayaraman2020revisiting}.

\paragraph{Secure multiparty computation.}
Secure multiparty computation (MPC) is a family of techniques that enable mutually distrustful parties to collaboratively compute a function of their distributed inputs without revealing those inputs. MPC techniques include \emph{garbled circuits}~\cite{yao1986generate} (which is most easily applied in the two-party case) and approaches based on \emph{secret sharing}~\cite{shamir1979share} (which naturally apply in the $n$-party case). MPC approaches have seen rapid improvement over the past 20 years, but scalability remains a challenge for practical deployments. In particular, most MPC protocols work best when the number of parties is small (e.g., 2 or 3), and costs grow at least quadratically with the number of parties. State-of-the-art protocols support significantly more parties: Wang et al.~\cite{wang2017global} reach 128 parties using a garbled circuits approach, and Chida et al.~\cite{chida2018fast} reach 110 parties using a secret sharing approach.

\paragraph{Threat model: central differential privacy.}
Most existing differentially private training algorithms, such as Abadi et al.'s, leverage \emph{central differential privacy}---they require the training data to be collected centrally (i.e. on a single server). The party that holds the data and runs the training algorithm is often called the \emph{data curator}, and in the central model, the data curator must be trusted. Central-model algorithms offer the best accuracy of known approaches, at the expense of requiring a trusted data curator.

\paragraph{Threat model: local differential privacy.}
The classical method to eliminate a trusted data curator is \emph{local differential privacy}~\cite{dwork2014algorithmic}, in which each participant adds noise to their own data before sending it to the data curator. Local differential privacy algorithms for gradient descent have been proposed, but for deep neural networks, this approach introduces too much noise to train useful models~\cite{bhowmick2018protection}. The major strength of local differential privacy is the threat model: privacy is assured for each participant, \emph{even if every other participant and the data curator act maliciously}. The local model of differential privacy has also been relaxed to the \emph{shuffle model}~\cite{cheu2019distributed, erlingsson2019amplification}, which lies between the local and central models but which has seem limited use in distributed machine learning.

\paragraph{Threat model: secure aggregation \& MPC.}
The difference in accuracy between the central and local models raises the question: can cryptography help us obtain the benefits of both, simultaneously? Several secure aggregation protocols have been proposed in the context of federated learning to answer this question in the affirmative. These approaches yield the \textbf{accuracy of the central model}, but \textbf{without a trusted data curator}. However, none offers a threat model as strong as local differential privacy---existing approaches require either a \textbf{semi-honest data curator}~\cite{bonawitz2017aggregation, mcmahan2017communication, truex2019hybrid} or \textbf{two non-colluding data curators}~\cite{DBLP:conf/nips/JayaramanW0G18}.

\subsection{Our Threat Model}

Our work targets a stronger threat model than previous work in differentially private distributed learning- specifically a \textbf{malicious data curator} and \textbf{malicious participants}, but with the assumption of an \textbf{honest majority} among the participants. The key insight behind this threat model is that \emph{each data owner is incentivized to protect his or her own data}, so the assumption of an honest majority among participants is likely to hold in practice.

Previous approaches that leverage MPC or secure aggregation provide privacy in the presence of only a very small number of corrupted parties (typically $O(1)$---see Table~\ref{fig:approaches}), because they involve the delegation of processing to a small number of designated parties (either a single server, or 2 or 3 computation parties that engage in an MPC protocol).

The assumption in these systems is that \emph{collusion is less likely} among the aggregators than among ordinary individuals---typically because they are operated by a large organization that would be harmed by allegations of malicious behavior.
%
However, the assumption of non-collusion between aggregators may not be reasonable in all settings---for example, even large organizations can be compromised by outside attackers, and many individuals will be unlikely to trust aggregators run by large organizations that have previously behaved maliciously or experienced data breaches.

Our threat model attempts to move as close as possible to the much stronger local model by improving collusion resistance, while maintaining high accuracy. The major difference between our threat model and that of the local model is our assumption of an honest majority among participants. As discussed in prior work~\cite{roth2019honeycrisp}, the actual number of malicious participants in a large-scale system deployment is likely to be just a few percent of the total.

\subsection{Challenges of MPC for Deep Learning}

Building MPC systems that are more resistant to collusion is challenging because most MPC protocols scale poorly with the number of parties~\cite{evans2017pragmatic}. Approaches based on garbled circuits are most easily applied in the two-party case; approaches based on secret sharing work for more parties, but communication scales quadratically with the number of parties. State-of-the-art systems that specifically target the many-party case have reached 128 parties~\cite{wang2017global, chida2018fast}.

The deep learning setting presents an additional challenge: the \emph{computation} associated with aggregating gradients is simple, but its \emph{dimensionality} is extremely high. Secure aggregation of gradients requires element wise summation of many vectors of dimension $k$, where $k$ is the number of trainable parameters in the model architecture. Our evaluation considers models with 550,000 parameters, and deployed (non-private) models in practice often have 10-100 \emph{million} parameters. The dimensionality of these gradients makes scalability of secure aggregation protocols especially challenging.




